Rapid evolution of [WC] stars in the Magellanic Clouds

We obtained new spectra of fourteen Magellanic Cloud planetary nebulae with the South African Large Telescope to determine heating rates of their central stars and to verify evolutionary models of post-asymptotic giant branch stars. We compared new spectra with observations made in previous years. Five planetary nebulae showed an increase in excitation over time. Four of their central stars exhibit [WC] features in their spectra, including three new detections. This raises the total number of [WC] central stars of PNe in the Magellanic Clouds to ten. We compared determined heating rates of the four [WC] central stars with the He-burning post-asymptotic giant branch evolutionary tracks and the remaining star with the H-burning tracks. Determined heating rates are consistent with the evolutionary models for both H and He-burning post-asymptotic giant branch stars. The central stars of the PNe that show the fastest increase of excitation are also the most luminous in the sample. This indicates that [WC] central stars in the Magellanic Clouds evolve faster than H-burning central stars, and they originate from more massive progenitors.

==> response.tex <==
Thank you for your comments. I have recomputed the PN models, which are constrained by observed diameters (if available) and absolute Hbeta fluxes. However, this did not modify derived parameters and heating rates significantly. I also added [OIII]/Hbeta ratios from Reid & Parker (2006), which I missed previously.

I rearranged the text and tried to describe the analysis methods more clearly. I also included more detailed description of error analysis.

In addition to model dependent luminosities I also provided model dependent final masses of the central stars obtained with the same method.

I also changed the classification of the new [WC] stars. The previous one based on wrong criteria. The new version does not include the histogram of the [WC] subtypes, since the statistics is very low.

The detalied description of the specific modifications is given below.


** Sect 1

Parg. 5:
1. While a PN central star may experience a post-AGB thermal pulse, this was not demonstrated by Paczynski (1970). Iben & Renzini (1983, ARA+A, 21, 271) pointed out (their Sect. 5.1.2) that the apparent late thermal pulse in Paczynski's model was an artifact of improper choices of inter-shell chemical and thermal structure. Schonberner (1979, A+Ap, 79, 108) is probably the first to demonstrate numerically the possibility of a post-AGB thermal pulse.  

- I changed the relevant reference.

** Sect 2

* Parg. 2:
2. Add a citation for the Robert Stobie Spectrograph. Perhaps Sheinis, A.I., et al. (2010, Proc. SPIE 7735, 1835) would be appropriate?

- I have already added two citations for the RSS previously (Kobulnicky et al. 2003; Burgh et al. 2003). The RSS was known as PFIS at that time.

* Parg. 3:
3. Clarify the slit orientation. That is, does a setting of 0 deg mean a north-south orientation?

-done

* Parg. 5:
4. Tables 1, 2, and 3 at the end of the paper give emission line intensities, presumably for a superset of the nebulae examined here. However, these tables are never called out in the text. Note that these table numbers overlap with tables that appear within the main body of the text: the observing log, the log of standard star observations, etc. If they are intended for a yet-to-be-created appendix, the numbering would be Table A1, A2, etc.

-I now clarified this, and corrected the table numbering. Also, I refer to the tables in the main text. Table 1 gives emission line intensities for all the PNe, while Table 2 gives the observed and modeled line intensities for the five PNe showing flux evolution.

** Sect. 3

* Parg. 1:
5. A citation is needed to support the assertions that a hydrogen-poor atmosphere indicates shell He burning, and that such stars show "wide and prominent stellar wind lines" in their spectra.

-Now I corrected this. H-poor atmosphere in a post-AGB star implies He burning, since no H is left. However, not all the H-poor CSPNs are [WC] stars, that was an imprecise statement.

* Parg. 2:
6. The author states that the presence of a C_III 5696 line of 1.9 Ang indicates a [WC 11] spectral type. In sect. 2 the author said the spectral resolution was about 800. That would imply instrumental linewidths of about 7 Ang. How was a FWHM of 1.9 Ang determined?

-That was my mistake. I have not measured FWHMs, but eqiuvalent widhts. The spectral classification by Acker & Neiner relies on equivalent widths. 

** Sect. 4

7. Although it would not greatly affect the conclusions, there is evidence that one member of the sample, SMP-LMC-104a, is a symbiotic star: see, e.g., the comments in Leisy & Dennefeld (2006, A+Ap, 456, 451) on the unphysical [O_III] temperature ([O_III] 4363 is likely elevated because of shocks) and the Fe features in the spectrum. TESS observations in MAST (https://mast.stsci.edu/portal/Mashup/Clients/Mast/Portal.html) show that the central source is variable on a timescale of days, with a periodic amplitude of a few percent.

- The [OIII] 5007 & 4959A lines have much lower critical densities than the [OIII] 4363A line, so for young PNe their ratio can be suppressed by high density. The variability of the central star could be also caused by pulsations (e.g. Handler, G., 2003, IAUS, 209, 237), wind variability or binarity.

* Parg. 5:
8. The author stated that the upper temperature limit used for the ionizing stars in the photoionization model was 50,000 K. One wonders if this limit is too low, at least for SMP31, where He_II 4686 emission is small but finite. Perhaps a higher T_eff would increase the modelled [O_III] 5007 flux?

-The HeII emission in SMP31 may be of stellar origin, since it also shows other stellar wind lines. The fits showed in Table A2 used were constrained by different emission lines. The modeled temperature for SMP31 is still well below 50kK.

9. There is no call-out to the table where the modeled and observed line intensities are observed (the last table in the paper, incorrectly labelled "Table 1." Was this table also intended for an appendix?

-I now refer to these tables in the text.

10. The author states that the nebular sizes are taken from the literature. Most sizes in the literature, if based on ground-based observations, are wrong. Those that are based on HST measurements are often good. Note that SMC-SMP-01 is unresolved at HST resolution, and SMP-LMC-31 is barely resolved. How would this affect the computed photoionization model? The author should be explicit about what sizes are adopted (presumably in Table 3), and the source of the measurement.

- I added the sizes. I constrained the models also with absolute Hbeta flux.

* Parg. 6:
11. For what epoch does the T_eff in Row 2 of Table 3 apply? How can the near perfect agreement in T_eff for all targets (37,000 K to within 900 K or so) be explained?     

- The temperature applies for 2013. Perhaps there is some observational bias. According to the photoionization model shown in Fig. 2, the [OIII]/Hbeta flux evolution is fastest near 37 kK.

12. I cannot follow the method from the description, but this paragraph is critical to understanding the central point of the paper. Presumably the author has the following as input:

 a. log L/L_o and T_eff from the literature (to which the author compares his results)
 b. log L/L_o and T_eff from photoionization models, at multiple epochs
 c. The time rate of change in T_eff at a particular T_eff, presumably referenced to the epoch of the observations presented here

- I now clarified this in the text. The rate of change in T_eff is an average value for the time span of observations. The value of log L/L_o is derived from the observed heating rate and the evolutionary model.

12.a. It is not clear what L_MOD is, how it, and the associated uncertainties, were determined.

12.b. It is not clear what is being determined by "interpolating evolution tracks. In any case, if the superior models of Miller Bertolami (2016) evolve faster and at a higher luminosity than those of Vassiliadis & Wood (1994), why were the V&W models interpolated for the four [WC] central stars?

- Only three He-burning models were computed by MB16 (including one late thermal pulse), which is not enough to interpolate the observed heating rates. I now clarified this in the text.

12.c. If the heating rates are used to determine the model-dependent luminosities from stellar evolution tracks, saying in Sect. 5, parg. 4 that "[t]he derived heating rates are consistent with the evolutionary models" sounds like circular reasoning. Significant clarification is needed.

-That was a simplification. We derived model-dependent luminosities from the heating rates. The heating rate is a very strong function of mass (and thus luminosity). We fitted the heating rates to the evolutionary tracks and derived (model dependent) luminosities.

####

** Sect. 5

* Parg. 2:
13. The author states "[t]he remaining six central stars may evolve too slowly to show significant evolution of the [O_III] 5007...." Please be more specific. All of these targets have some measure of the (log L, T_eff), which maps directly to a stellar mass on some evolution track, and therefore also to a heating rate. The question is given the implied heating rates, would these be detectable?

-I estimated that the heating rates of 5-10 kK would be detectable, so the remaining central stars are most likely less massive than those which show the evolution of [OIII]/Hbeta flux. 

* Parg. 7:
14. It would be more prudent to say that the correlation of rapid inferred evolution in stellar T_eff with [WC] emission "implies," rather than "indicates," high stellar mass.

-done

* Parg. 8:
15. It is more appropriate to say that the rapid inferred heating rate for the Galactic PNe M1-11 and M1-12 "suggests" (rather then "indicates") that the lifetime of PNe with [WC] central stars is shorter.

-done

** Figure 2

16. This figure has marginal scientific merit, and could be omitted.

- Done

** Table 3

17. It is very hard to tell which quantities come from which references. A separate column labelled "Ref" for each PN (rather than a single row for all references) would make it much more clear.

- I corrected this table.

18. Please explain the following:
 - Two rows have the name "L/L_o(H I)" but have different values for one object.
 - Two rows have the name "log L_SED/L_o" but have different values for two objects.
 - How are uncertainties determined for the heating rate (row 2)?
 - What do the uncertainties mean for a modelled luminosity (L_MOD)?
Perhaps these questions would be resolved if Table 3 were re-organized to make the references more clear (see above point).

-I rearranged Table 3. I also added the discussion of the derived uncertainties in the text.


** Table 4

19. Two of the sources (SMP-LMC-64 and SMP-LMC-104a) have no listed values for any of the quantities. Was this information accidentally omitted? If not, they should be removed from the table.

- These values were not derived in the literature. I deleted these PNe.

** Emission line intensity tables

20. Explain in the table caption the meaning of the delta-I columns. Presumably this is the change in emission line intensity relative to some reference epoch/observer. But then which is the reference epoch?

-Now the caption describes the content of the table. delta-I are uncertainties.

21. Table notes should be added to indicate which emission features are likely to be of stellar origin.

-I added superscripts indicating stellar origin.

22. There are multiple instances where the table entries are clearly wrong. A few obvious examples are noted below. These tables need to be reviewed carefully for accuracy.

 - The intensities for SMP_31 for [N_II] 6548 have unexpectedly tiny values w.r.t. the [N_II] 6583 emission. And the H-alpha values are unphysical. It looks as if intensities were placed in the wrong rows.
- Similar comments apply to the instensities for MG-SMP-08: The C_III 4651 and He_II 4686 values are obviously wrong, as are those for [N_II] 6548.

-C_III 4651 and He_II 4686 in MG-SMP-08 are of stellar origin (I added a relevant superscripts in the table). I also corrected the order of the rows for SMP 31.

23. The header row should give the full PN designation (i.e., including the host galaxy: LMC or SMC) for clarity.

-I corrected this.

####. Manuscript errors

** Abstract

M1. In the first sentence, it would be more accurate to say that new spectra were "obtained" rather than "derived."

- corrected

M2. The author should clarify that the sentence: "This raises the total number of [WC] stars in..." refers to WC central stars of planetary nebulae.

- corrected

** Sect 1

M3. The author should clarify that "Stars with an initial mass of 1--8 M_o form a carbon-oxygen core." refers to post-main sequence stars.

-done

* Parg. 3:
M4. Correct the grammar: "After a star ejects most of..." not "when."

-done

* Parg. 4:
M5. Clarify the wording: Post-AGB stars cross the H-R diagram "at constant luminosity" rather than "horizontally."

-done

** Sect. 3

Parg. 1:
M6. Two sentences are missing a leading article: "A hydrogen poor atmosphere..." and "A hydrogen rich atmosphere...".

-done

** Sect. 5

* Parg. 3
Figure 4 is called out in the text before Fig. 3.

-corrected

* Parg. 8:
M7. "born rate" -> "birth rate"

-done


